Achieving Flexible and Secure Authentication with Strong Privacy in Decentralized Networks

Anonymous credentials (ACs) are a crucial cryptographic tool for privacy-preserving authentication in decentralized networks, allowing holders to prove eligibility without revealing their identity. However, a major limitation of standard ACs is the disclosure of the issuer's identity, which can leak sensitive contextual information about the holder. Issuer-hiding ACs address this by making a credential's origin indistinguishable among a set of approved issuers. Despite this advancement, existing solutions suffer from practical limitations that hinder their deployment in decentralized environments: unflexible credential models that restrict issuer and holder autonomy, flawed revocation mechanisms that compromise security, and weak attribute hiding that fails to meet data minimization principles. This paper introduces a new scheme called IRAC to overcome these challenges. We propose a flexible credential model that employs vector commitments with a padding strategy to unify credentials from heterogeneous issuers, enabling privacy-preserving authentication without enforcing a global static attribute set or verifier-defined policies. Furthermore, we design a secure decentralized revocation mechanism where holders prove non-revocation by demonstrating their credential's hash lies within a gap in the issuer's sorted revocation list, effectively decoupling revocation checks from verifier policies while maintaining issuer anonymity. IRAC also strengthens attribute hiding by utilizing zk-SNARKs and vector commitments, allowing holders to prove statements about their attributes without disclosing the attributes themselves or the credential structure. Security analysis and performance evaluations demonstrate its practical feasibility for decentralized networks, where presenting a credential can be finished in 1s.

==> sections/bios.tex <==
 \begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{figure/photos/xiebin}}]{Bin Xie} received the BSc and MSc degrees from Northeastern University, Shenyang, China and Chongqing University, Chongqing, China, respectively. He is currently working toward the PhD degree in the Department of Computing, The Hong Kong Polytechnic University. His research interests include authentication and privacy protection.
 \end{IEEEbiography}


 
% \begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{figure/photos/zhengtianyu}}]{Tianyu Zheng} received the B.E. degree in 2020
% and M.E. degree in 2022, both from the Southeast
% University, China. He is currently a Ph.D. student
% from the Hong Kong Polytechnic University, Hong
% Kong. His research interests include applied cryptography, zero-knowledge proofs, RingCT protocol,
% and zkSNARKs.
%  \end{IEEEbiography}

 \begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{figure/photos/songrui}}]{Rui Song} received the BSc and MSc degrees in cyber security from Southeast University, Nanjing,
China. He is currently working toward the PhD degree with the Department of Computing, The Hong Kong Polytechnic University under the supervision of prof. Bin Xiao. His research interests include blockchain systems and data privacy.
\end{IEEEbiography}

% \begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{figure/photos/xiaotiedeng}}]{Xiaotie Deng}(Fellow, IEEE) received the BSc degree from Tsinghua University, the MSc degree from the Chinese Academy of Sciences, and the PhD degree from Stanford University, in 1989. He is currently a chair professor with Peking University. He has taught with Shanghai Jiaotong University, the University of Liverpool, the City University of Hong Kong, and York University. His current research interests include algorithmic game theory, with applications to Internet economics and finance. He is an ACM fellow for his contribution to the interface of algorithms and game theory and an IEEE fellow for his contributions to computing in partial information and interactive environments.
% \end{IEEEbiography}
 

 \begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{figure/photos/xiaobin}}]{Bin Xiao} (Fellow, IEEE) is a professor at the Department of Computing, the Hong Kong Polytechnic University, Hong Kong. Prof. Xiao received B.Sc and M.Sc degrees in Electronics Engineering from Fudan University, China, and a Ph.D. degree in computer science from the University of Texas at Dallas, USA. His research interests include AI security and privacy, data privacy, Web3, and blockchain systems. He published more than 200 technical papers in international top journals and conferences. He is currently an Associate Editor of the IEEE Transactions on Cloud Computing. He has been the associate editor of the IEEE Internet of Things Journal, IEEE Transactions on Network Science and Engineering, and Elsevier Journal of Parallel and Distributed Computing. He has been the chair of the IEEE ComSoc CISTC committee from 2024 to 2025 and the IEEE ComSoc Distinguished Lecturer from 2023 to 2024. He has been the program co-chair of IEEE CNS2025, track co-chair of IEEE ICDCS2022, the symposium track co-chair of IEEE Globecom 2024, ICC2020, ICC 2018, and Globecom 2017, and the general chair of IEEE SECON 2018. 
% He is the vice chair of IEEE ComSoc CISTC committee. He has been the track co-chair of IEEE ICDCS 2022, symposium track co-chair of IEEE ICC 2020, ICC 2018 and Globecom 2017, and the general chair of IEEE SECON 2018.
 \end{IEEEbiography}



==> sections/security-analysis.tex <==
\section{Security Analysis}
\label{sec:security-analysis}
to do...
